Optimising Density Computations in Probabilistic Programs via Automatic Loop Vectorisation

Probabilistic programming languages (PPLs) are a popular tool for high-level modelling across many fields. They provide a range of algorithms for probabilistic inference, which analyse models by learning their parameters from a dataset or estimating their posterior distributions. However, probabilistic inference is known to be very costly. One of the bottlenecks of probabilistic inference stems from the iteration over entries of a large dataset or a long series of random samples. Vectorisation can mitigate this cost, but manual vectorisation is error-prone, and existing automatic techniques are often ad-hoc and limited, unable to handle general repetition structures, such as nested loops and loops with data-dependent control flow, without significant user intervention. To address this bottleneck, we propose a sound and effective method for automatically vectorising loops in probabilistic programs. Our method achieves high throughput using speculative parallel execution of loop iterations, while preserving the semantics of the original loop through a fixed-point check. We formalise our method as a translation from an imperative PPL into a lower-level target language with primitives geared towards vectorisation. We implemented our method for the Pyro PPL and evaluated it on a range of probabilistic models. Our experiments show significant performance gains against an existing vectorisation baseline, achieving $1.1$--$6\times$ speedups and reducing GPU memory usage in many cases. Unlike the baseline, which is limited to a subset of models, our method effectively handled all the tested models.

==> sections/fig-trg2l-def-sem.tex <==
\begin{figure}[t]
\newcommand{\vspacesem}{1.8ex}
\[
\begin{array}{c}
\infer{
    (x^\lreal := \code{fetch}(I)), D, \sigma, A \Downarrowtt \sigma', \pi_\emptyset[y^{\tau\dagger} \mapsto B^A_0 : y^{\tau\dagger} \in \FV(I)][x^{\lreal} : B^A_1], T'
}{
    (x^\lreal := \code{fetch}(I)), D, \sigma, A \Downarrowt \sigma', T'
}
\\[\vspacesem]
\infer{
    \code{score}(E), D, \sigma, A \Downarrowtt \sigma', \pi_\emptyset[y^{\tau\dagger} \mapsto B^A_0 : y^{\tau\dagger} \in \FV(E)], T'
}{
    \code{score}(E), D, \sigma, A \Downarrowt \sigma', T'
}
\\[\vspacesem]
\infer{
    (x^\lintt := Z), D, \sigma, A \Downarrowtt \sigma', \pi_\emptyset[y^{\tau\dagger} \mapsto B^A_0 : y^{\tau\dagger} \in \FV(Z)][x^{\lintt} : B^A_1], T'
}{
    (x^\lintt := Z), D, \sigma, A \Downarrowt \sigma', T'
}
\\[\vspacesem]
\infer{
    (x^\lreal := E), D, \sigma, A \Downarrowtt \sigma', \pi_\emptyset[y^{\tau\dagger} \mapsto B^A_0 : y^{\tau\dagger} \in \FV(E)][x^{\lreal} : B^A_1], T'
}{
    (x^\lreal := E), D, \sigma, A \Downarrowt \sigma', T'
}
\\[\vspacesem]
\infer{
    \code{skip}, D, \sigma, A \Downarrowtt \sigma, \pi_\emptyset, T^z_A
}{}
\qquad
\infer{
    (C_1;C_2), D, \sigma, A \Downarrowtt \sigma'', \pi'[\pi''], (T' \oplus T'')
}{
    C_1, D, \sigma, A \Downarrowtt \sigma', \pi', T'
    &
    C_2, D, \sigma', A \Downarrowtt \sigma'', \pi'', T''
}
\\[\vspacesem]
\infer{
    (\code{ifz}\ Z\ C_1\ C_2), D, \sigma, A \Downarrowtt \sigma'', \pi_\emptyset[y^{\tau\dagger} \mapsto B^A_0 : y^{\tau\dagger} \in \FV(Z)][\pi'][\pi''], (T' \oplus T'')
}{
    \begin{array}{ll}
    A_1 = \{i \in A : \db{Z}(\sigma,i) = 0\}
    & 
    C_1, D, \sigma, A_1 \Downarrowtt \sigma', \pi', T'
    \\[0.5ex]
    A_2 = \{i \in A : \db{Z}(\sigma,i) \neq 0\}
    &
    C_2, D, \sigma', A_2 \Downarrowtt \sigma'', \pi'', T''
    \end{array}
}
\\[\vspacesem]
\infer{
    (\code{for}\ x^\lintt \ \code{in} \ \code{range}(n_+)\ \code{do}\ C), D, \sigma, A
    \Downarrowtt \sigma_{n_+}, \pi'_{n_+}, \bigoplus_{k = 1}^{n_+} T_{k}
}{
    \begin{array}{ll}
    \sigma_0 = \sigma
    \quad
    C, D, \sigma_k[x^\lintt : [i \mapsto k \, :\, i \in A]], A \Downarrowtt \sigma_{k+1}, \pi_{k+1}, T_{k+1}
    \\
    \pi'_0 = \pi_\emptyset
    \quad
    \pi'_{k+1} = \pi'_k [\pi_{k+1}]
    \quad
    \text{for all $k \in \{0,{...}\,,n_+{-}1\}$}
    \end{array}
}
\\[\vspacesem]
\infer{
    (x^{\lintt} := \code{lookup\_index}(\alpha)), D, \sigma, A \Downarrowtt \sigma', \pi_\emptyset[x^{\lintt} : B^A_1], T'
}{
    (x^{\lintt} := \code{lookup\_index}(\alpha)), D, \sigma, A \Downarrowt \sigma', T'
}
\\[\vspacesem]
\infer{
    (\code{extended\_loop\_with\_shift}(\alpha, n_+)\ C), D, \sigma, A 
    \Downarrowtt
    \sigma_{m+1}\langle\rho\rangle, \pi''_{m+1}|_A, T
}{
    \begin{array}{ll}
    \alpha \not\in \dom(i) \text{ for all $i \,{\in}\, A$}
    \quad
    A' = \{ i \,{\concat}\, [(\alpha,k)] : i \,{\in}\, A,\, k \,{\in}\, \{0,{...}\,,n_+{-}1\} \}
    \\[0.5ex]
    0 \leq m < n_+ {-} 1
    \quad
    \sigma_0 = \sigma
    \quad
    \text{for all $\ell \in \{0,{...}\,,m-1\}$}
    \\[0.5ex]
    C, D, \sigma_\ell\langle\rho_\alpha\rangle, A' \Downarrowtt \sigma_{\ell+1}, \pi_{\ell+1}, T_{\ell+1}
    \quad
    \fixcheck(\sigma_\ell\langle\rho_\alpha\rangle, \sigma_{\ell+1}\langle\rho_\alpha\rangle, \pi_{\ell+1}, A') = 0
    \\[0.5ex]
    C, D, \sigma_m\langle\rho_\alpha\rangle, A' \Downarrowtt \sigma_{m+1}, \pi_{m+1}, T_{m+1}
    \quad
    \fixcheck(\sigma_m\langle\rho_\alpha\rangle, \sigma_{m+1}\langle\rho_\alpha\rangle, \pi_{m+1}, A') = 1
    \\[0.5ex]
    \pi_{n+1}' = \pi_{n+1}\langle\rho_\alpha\rangle^{-(n+1)}
    \quad
    \pi_0'' = \pi_\emptyset
    \quad
    \pi_{n+1}'' = \pi_n''[\pi_{n+1}']
    \quad
    \text{for all $n \in \{0,{...}\,,m\}$}
    \\[0.5ex]
    \rho = [i \concat [(\alpha, n_+{-}1)] \mapsto i : i \in A]
    \quad
    T = [i \mapsto \sum_{0 \leq k < n_+} T_{m+1}(i \concat [(\alpha,k)]) : i \in A]     
    \end{array}
}
\\[\vspacesem]
\infer{
    (\code{extended\_loop\_with\_shift}(\alpha, n_+)\ C), D, \sigma, A 
    \Downarrowtt
    \sigma_{n_+}\langle\rho\rangle, \pi''_{n_+}|_A, T
}{
    \begin{array}{ll}
    \alpha \not\in \dom(i) \text{ for all $i \,{\in}\, A$}
    \quad
    A' = \{ i \,{\concat}\, [(\alpha,k)] : i \,{\in}\, A,\, k \,{\in}\, \{0,{...}\,,n_+{-}1\} \}
    \\[0.5ex]
    \sigma_0 = \sigma
    \quad
    \text{for all $\ell \in \{0,{...}\,,n_+{-}2\}$}
    \\[0.5ex]
    C, D, \sigma_\ell\langle\rho_\alpha\rangle, A \Downarrowtt \sigma_{\ell}, \pi_{\ell}, T_{\ell}
    \quad
    \fixcheck(\sigma_\ell\langle\rho_\alpha\rangle, \sigma_{\ell}\langle\rho_\alpha\rangle, \pi_{\ell}, A) = 0
    \\[0.5ex]
    C, D, \sigma_{n_+{-}1}\langle\rho_\alpha\rangle, A \Downarrowtt \sigma_{n_+}, \pi_{n_+}, T_{n_+}
    \\[0.5ex]
    \pi_{n+1}' = \pi_{n+1}\langle\rho_\alpha\rangle^{-(n+1)}
    \quad
    \pi_0'' = \pi_\emptyset
    \quad
    \pi_{n+1}'' = \pi_n''[\pi_{n+1}']
    \quad
    \text{for all $n \in \{0,{...}\,,n_+{-}1\}$}
    \\[0.5ex]
    \rho = [i \concat [(\alpha, n_+{-}1)] \mapsto i : i \in A]
    \quad
    T = [i \mapsto \sum_{0 \leq k < n_+} T_{n_+}(i \concat [(\alpha,k)]) : i \in A]   
    \end{array}
}
\end{array}
\]
\vspace{-1em}
\caption{Semantics of commands in the relaxed target language.}
\label{fig:semantics-commands-target-language-appendix}
\end{figure}

==> sections/fixed-point-condition.tex <==
\section{Relaxing Fixed-point Condition}
\label{sec:relaxed-fixed-point-condition}

A \emph{flag} $\pi$ is a function from variables to finite partial maps from indices to $0$ or $1$:
\begin{align*}
    \pi &: \Var \to [\Index \finpartialto \{0,1\}].
\end{align*}
Intuitively, $\pi$ records $0$ or $1$ indicating whether the first occurrence of each variable during the execution within a scope of an index
is read in an expression or written by an assignment.
We define $\Flag$ as the set of all flags.
Let $\pi_\emptyset = [x^{\tau\dagger} \mapsto [] : x^{\tau\dagger} \in \Var]$ be an empty flag.
For finite partial maps $B$ and $B'$ from indices to $0$ or $1$, we define the update operator $B[B']$ by
\begin{align*}
    B[B'](i) &=
    \begin{cases}
        B(i) & \text{if } i \in \dom(B), \\
        B'(i) & \text{otherwise}.
    \end{cases}
\end{align*}
We define the update operator of a flag $\pi$ by $B$ for a variable $x^{\tau\dagger}$ as follows:
\begin{align*}
    \pi[x^{\tau\dagger} : B](y^{\tau'\dagger}) &=
    \begin{cases}
        \pi(x^{\tau\dagger})[B] & \text{if } y^{\tau\dagger} \equiv x^{\tau\dagger}, \\
        \pi(y^{\tau'\dagger}) & \text{otherwise}.
    \end{cases}
\end{align*}
Let $h$ be a finite partial map from variables to finite partial maps from indices to $0$ or $1$.
We define the update operator of a flag $\pi$ by $h$, $\pi[h]$,
by updating all the partial maps assigned to each variable in $\pi$ by those in $h$:
\begin{align*}
    \pi[h](x^{\tau\dagger}) &=
    \begin{cases}
    \pi(x^{\tau\dagger})[h(x^{\tau\dagger})] & \text{if } x^{\tau\dagger} \in \dom(h), \\
    \pi(x^{\tau\dagger}) & \text{otherwise}.
    \end{cases}
\end{align*}
For $\pi, \pi' \in \Flag$, we define the partial order $\pi \leq \pi'$ by
\begin{align*}
    \pi \leq \pi' &\iff \forall x^{\tau\dagger} \in \Var.\,
    i \in \dom(\pi(x^{\tau\dagger})) \implies
    i \in \dom(\pi'(x^{\tau\dagger})) \land \pi(x^{\tau\dagger})(i) = \pi'(x^{\tau\dagger})(i).
\end{align*}
When $\pi \leq \pi'$, we define $\pi' \setminus \pi \in \Flag$ by
\begin{align*}
    (\pi' \setminus \pi)(x^{\tau\dagger}) &=
    [i \mapsto \pi'(x^{\tau\dagger})(i) : i \in \dom(\pi'(x^{\tau\dagger})) \setminus \dom(\pi(x^{\tau\dagger}))]
    \quad \text{for all } x^{\tau\dagger} \in \Var.
\end{align*}
Let $\FV(Z)$, $\FV(E)$, and $\FV(I)$ be the sets of free variables in an integer expression $Z$, a real expression $E$, and an index expression $I$, respectively.

For a set of indices $L \subseteq \Index$ and two tensors $T_0, T_1 \in \Tensor_{\db{\tau}}$,
we define $T_0 =_L T_1$ by
\begin{align*}
    T_0 =_L T_1 \iff
    T_0 [\WTensor_{\db{\tau}}(\Delta_L)] T_1 \iff
    \extend(T_0)(i) = \extend(T_1)(i)
    \quad \text{for all } i \in L.
\end{align*}
Let $\IndexInj$ be a set of injective partial maps from $\Index$ to $\Index$.
For $\pi \in \Flag$ and $\rho \in \IndexInj$,
we define $\pi\langle\rho_{\alpha}\rangle$ by considering $\pi$ as a state in $\State_{\textit{tgt}}$ and applying the copy operation.
We denote $\rho_{\alpha} \in \IndexInj$ as the partial map defined in the semantics of the command $\code{shift}(\alpha)$ in the target language.
It also depends on $A$, but we omit $A$ in the notation for simplicity, as it is clear from the context.
For $n \geq 1$, we define $\pi\langle\rho_{\alpha}\rangle^{-n} \in \Flag$ as follows:
\begin{align*}
    \pi\langle\rho_{\alpha}\rangle^{-1}(x^{\tau\dagger})(i) &=
    \begin{cases}
        \pi(x^{\tau\dagger})(\rho_{\alpha}(i)) & \text{if } i \in A, \\
        \pi(x^{\tau\dagger})(i) \sqcap \pi(x^{\tau\dagger})(\rho(i)) & \text{if } i \in A^c \cap \dom(\rho_{\alpha}), \\
        \pi(x^{\tau\dagger})(i) & \text{otherwise},
    \end{cases} \\
    \pi \langle\rho_{\alpha}\rangle^{-n}
    &= (\pi \langle\rho_{\alpha}\rangle^{-(n-1)})\langle\rho_{\alpha}\rangle^{-1}
    \quad \text{for } n > 1.
\end{align*}
Here, for $b_1, b_2 \in \{0, 1, \text{undefined}\}$,
\begin{align*}
b_1 \sqcap b_2 =
\begin{cases}
b_1 & \text{if } b_1 = b_2, \\
\text{undefined} & \text{otherwise}.
\end{cases}
\end{align*}
For $A \in \FAntiChain$, we define the restricted flag $\pi|_A \in \Flag$ by $\pi|_A(x^{\tau\dagger}) = \pi(x^{\tau\dagger})|_A$
for any $x^{\tau\dagger} \in \Var$.

We define the semantics of commands in the relaxed target language by the big-step relation
\begin{align*}
    C, D, \sigma, A \Downarrowtt \sigma', \pi, T,
\end{align*}
where $C$ is a command in the relaxed target language, $D \in \RDB$, $\sigma, \sigma' \in \State_{\textit{tgt}}$,
$A \in \FAntiChain$, $\pi \in \Flag$, and $T \in \Tensor_{\R}$.
The rules for the semantics are given in \Cref{fig:semantics-commands-target-language-appendix}.
Here, $\fixcheck(\sigma, \sigma', \pi, A)$ is defined as follows:
\begin{align*}
    \fixcheck(\sigma, \sigma', \pi, A) &=
    \begin{cases}
        1 & \text{if}\ \ \forall x^{\tau\dagger} \in \Var.\, \sigma(x^{\tau\dagger}) =_{A \setminus \{i \,:\, \pi(x^{\tau\dagger})(i) = 1\}} \sigma'(x^{\tau\dagger}), \\
        0 & \text{otherwise}.
    \end{cases}
\end{align*}
Also, for $S \subseteq \Var$ and $A \in \FAntiChain$,
we use the notations $B^A_0, B^A_1$ defined as follows:
\begin{align*}
    B^A_0 = [i \mapsto 0 : i \in A], \quad
    B^A_1 = [i \mapsto 1 : i \in A].
\end{align*}

\input{sections/fig-trg2l-def-sem}

\begin{lemma}
\label{lem:relaxed-fixed-point-expression}
Let $Z$ be an integer expression, $E$ be a real expression, $I$ be an index expression.
Let $\sigma_0, \sigma_1 \in \State_{\textit{tgt}}$ and $A \in \FAntiChain$.
The following statements hold:
\begin{enumerate}[itemsep=5pt]
    \item If $\,\forall y^{\tau\dagger} \in \FV(Z).\, \sigma_0(y^{\tau\dagger}) =_A \sigma_1(y^{\tau\dagger})$,
    then $\db{Z}(\sigma_0, i) = \db{Z}(\sigma_1, i)$ for all $i \in A$.
    \item If $\,\forall y^{\tau\dagger} \in \FV(E).\, \sigma_0(y^{\tau\dagger}) =_A \sigma_1(y^{\tau\dagger})$,
    then $\db{E}(\sigma_0, i) = \db{E}(\sigma_1, i)$ for all $i \in A$.
    \item If $\,\forall y^{\tau\dagger} \in \FV(I).\, \sigma_0(y^{\tau\dagger}) =_A \sigma_1(y^{\tau\dagger})$,
    then $\db{I}(\sigma_0, i) = \db{I}(\sigma_1, i)$ for all $i \in A$.
\end{enumerate}
\end{lemma}

The following lemma states that if a command in the relaxed target language is executed from two states
with which the relaxed fixed-point condition is satisfied, then the command produces the same state, flag, and tensor.
\begin{lemma}
\label{lem:relaxed-fixed-point-command}
Let $C$ be a command in the relaxed target language, $D \in \RDB$, $\sigma_0, \sigma_1, \sigma_0', \sigma_1' \in \State_{\textit{tgt}}$,
$A \in \FAntiChain$, $\pi_0, \pi_1, \pi \in \Flag$, and $T_0, T_1 \in \Tensor_{\R}$.
Suppose $\sigma_0$ and $\sigma_1$ are $A$-states, $\pi_0 \leq \pi$, and $\dom(\pi) \subseteq A$. If
\begin{align*}
    C, D, \sigma_0, A \Downarrowtt \sigma_0', \pi_0, T_0,
    \quad
    C, D, \sigma_1, A \Downarrowtt \sigma_1', \pi_1, T_1,
    \quad \text{and} \quad
    \fixcheck(\sigma_0, \sigma_1, \pi, A) = 1,
\end{align*}
then we have
\begin{align*}
\fixcheck(\sigma_0', \sigma_1', \pi \setminus \pi_0, A) = 1,
\quad
\pi_0 = \pi_1,
\quad \text{and} \quad
T_0 = T_1.
\end{align*}
\end{lemma}
\begin{proof}
    The proof is by induction on the structures of $C$.
    \begin{itemize}[itemsep=5pt]
    \item {\bf Case of $C \equiv (x^\lintt := Z)$ and $C \equiv (x^\lreal := E)$}: \\
        Clearly, $\pi_0 = \pi_1$ and $T_0 = T_1 = T^z_A$.
        For $y^{\tau\dagger} \in \FV(Z)$ or $y^{\tau\dagger} \in \FV(E)$,
        by the semantics of the assignment, we have $\pi_0(y^{\tau\dagger})(i) = 0$ for all $i \in A$.
        This implies $\pi(y^{\tau\dagger})(i) = 0$ for all $i \in A$ since $\pi_0 \leq \pi$.
        Hence, $A \setminus \{i : \pi(y^{\tau\dagger})(i) = 1\} = A$,
        and by the condition of $\fixcheck$, we have
        $\sigma_0(y^{\tau\dagger}) =_A \sigma_1(y^{\tau\dagger})$.
        By \Cref{lem:relaxed-fixed-point-expression}, we have
        \begin{align*}
        \db{Z}(\sigma_0, i) = \db{Z}(\sigma_1, i)
        \quad \text{or} \quad
        \db{E}(\sigma_0, i) = \db{E}(\sigma_1, i)
        \end{align*}
        for all $i \in A$, which results in $\sigma_0' = \sigma_1'$.
    \item {\bf Case of $C \equiv \code{skip}$}: \\
        Clearly, $\pi_0 = \pi_1 = \pi_\emptyset$ and $T_0 = T_1 = T^z_A$.
        Since $\sigma_0' = \sigma_0$, $\sigma_1' = \sigma_1$, and $\pi \setminus \pi_0 = \pi$,
        we have $\fixcheck(\sigma_0', \sigma_1', \pi \setminus \pi_0, A) = 1$.
    \item {\bf Case of $C \equiv (x^\lreal := \code{fetch}(I))$}: \\
        This is similar to the case of $C \equiv (x^\lreal := E)$.
    \item {\bf Case of $C \equiv (\code{score}(E))$}: \\
        This is similar to the case of $C \equiv (x^\lreal := E)$.
    \item {\bf Case of $C \equiv (x^\lintt := \code{lookup\_index}(\alpha))$}: \\
        This is similar to the case of $C \equiv (x^\lintt := Z)$.
    \item {\bf Case of $C \equiv (C_1;C_2)$}: \\
        By the semantics of $(C_1;C_2)$, there exist $\sigma_0'', \sigma_1'' \in \State_{\textit{tgt}}$,
        and $\pi_0', \pi_1', \pi_0'', \pi_1'' \in \Flag$,
        and $T_0', T_1', T_0'', T_1'' \in \Tensor_{\R}$ such that
        \begin{align*}
        C_1, D, \sigma_0, A \Downarrowtt \sigma_0'', \pi_0'', T_0'',
        \quad
        C_2, D, \sigma_0'', A \Downarrowtt \sigma_0', \pi_0', T_0',
        \quad
        \pi_0 = \pi_0''[\pi_0'],
        \quad
        T_0 = T_0'' \oplus T_0', \\
        C_1, D, \sigma_1, A \Downarrowtt \sigma_1'', \pi_1'', T_1'',
        \quad
        C_2, D, \sigma_1'', A \Downarrowtt \sigma_1', \pi_1', T_1',
        \quad
        \pi_1 = \pi_1''[\pi_1'],
        \quad
        T_1 = T_1'' \oplus T_1'.
        \end{align*}
        Since $\pi_0'' \leq \pi_0 \leq \pi$, by the induction hypothesis for $C_1$, we have
        \begin{align*}
        \fixcheck(\sigma_0'', \sigma_1'', \pi \setminus \pi_0'', A) = 1,
        \quad
        \pi_0'' = \pi_1'',
        \quad
        T_0'' = T_1''.
        \end{align*}
        Since $(\pi \setminus \pi_0'') \leq (\pi \setminus \pi_0'')[\pi_0']$,
        we also have
        \begin{align*}
        \fixcheck(\sigma_0'', \sigma_1'', (\pi \setminus \pi_0'')[\pi_0'], A) = 1.
        \end{align*}
        By the induction hypothesis for $C_2$, since $\pi_0' \leq (\pi \setminus \pi_0'')[\pi_0']$, we have
        \begin{align*}
        \fixcheck(\sigma_0', \sigma_1', (\pi \setminus \pi_0'')[\pi_0'] \setminus \pi_0', A) = 1,
        \quad
        \pi_0' = \pi_1',
        \quad
        T_0' = T_1'.
        \end{align*}
        Simple calculations give
        \begin{align*}
        \fixcheck(\sigma_0', \sigma_1', \pi \setminus \pi_0, A) = 1,
        \quad
        \pi_0 = \pi_1,
        \quad \text{and} \quad
        T_0 = T_1
        \end{align*}
        since $(\pi \setminus \pi_0) = (\pi \setminus (\pi_0''[\pi_0']))
        = ((\pi \setminus \pi_0'')[\pi_0'] \setminus \pi_0')$, as required.
    \item {\bf Case of $C \equiv (\code{ifz}\ Z\ C_1\ C_2)$}: \\
        For $y^{\tau\dagger} \in \FV(Z)$, by the semantics of the if-then-else command,
        we have $\pi_0(y^{\tau\dagger})(i) = 0$ for all $i \in A$.
        This implies $\pi(y^{\tau\dagger})(i) = 0$ for all $i \in A$ since $\pi_0 \leq \pi$.
        Hence, $A \setminus \{i : \pi(y^{\tau\dagger})(i) = 1\} = A$,
        and by the condition of $\fixcheck$, we have
        $\sigma_0(y^{\tau\dagger}) =_A \sigma_1(y^{\tau\dagger})$.
        By \Cref{lem:relaxed-fixed-point-expression}, we have
        \begin{align*}
        \db{Z}(\sigma_0, i) = \db{Z}(\sigma_1, i)
        \end{align*}
        for all $i \in A$.
        Thus, both executions of the if-then-else command take the same branch.
        Let 
        \begin{align*}
            h_0 = [y^{\tau\dagger} \mapsto B^A_0 : y^{\tau\dagger} \in \FV(Z)],
            \quad
            A_1 = \{i \in A : \db{Z}(\sigma_0,i) = 0\},
            \quad
            A_2 = \{i \in A : \db{Z}(\sigma_0,i) \neq 0\}.
        \end{align*}
        By the semantics of $(\code{ifz}\ Z\ C_1\ C_2)$, there exist $\sigma_0'', \sigma_1'' \in \State_{\textit{tgt}}$,
        and $\pi_0', \pi_1', \pi_0'', \pi_1'' \in \Flag$,
        and $T_0', T_1', T_0'', T_1'' \in \Tensor_{\R}$ such that
        \begin{align*}
        C_1, D, \sigma_0, A_1 \Downarrowtt \sigma_0'', \pi_0'', T_0'',
        \quad
        C_2, D, \sigma_0'', A_2 \Downarrowtt \sigma_0', \pi_0', T_0',
        \quad
        \pi_0 = \pi_\emptyset[h_0][\pi_0''][\pi_0'],
        \quad
        T_0 = T_0'' \oplus T_0', \\
        C_1, D, \sigma_1, A_1 \Downarrowtt \sigma_1'', \pi_1'', T_1'',
        \quad
        C_2, D, \sigma_1'', A_2 \Downarrowtt \sigma_1', \pi_1', T_1',
        \quad
        \pi_1 = \pi_\emptyset[h_0][\pi_1''][\pi_1'],
        \quad
        T_1 = T_1'' \oplus T_1'.
        \end{align*}
        Let $\pi' = \pi \setminus \pi_\emptyset[h_0]$.
        For any $x^{\tau\dagger} \in \Var$,
        since all indices are mapped to $0$ in $\pi_\emptyset[h_0](x^{\tau\dagger})$,
        \begin{align*}
        \{i : \pi'(x^{\tau\dagger})(i) = 1\} = \{i : \pi(x^{\tau\dagger})(i) = 1\}.
        \end{align*}
        This implies $\fixcheck(\sigma_0, \sigma_1, \pi', A) = 1$,
        and $\fixcheck(\sigma_0, \sigma_1, \pi'[\pi_0''], A_1) = 1$.
        Since $\pi_0'' \leq \pi'[\pi_0'']$, by the induction hypothesis for $C_1$, we have
        \begin{align*}
        \fixcheck(\sigma_0'', \sigma_1'', \pi'', A_1) = 1,
        \quad
        \pi_0'' = \pi_1'',
        \quad
        T_0'' = T_1''
        \end{align*}
        where $\pi'' = (\pi'[\pi_0''] \setminus \pi_0'')$.
        We claim $\fixcheck(\sigma_0'', \sigma_1'', \pi'', A) = 1$.
        To see this, let $x^{\tau\dagger} \in \Var$, and
        \begin{align*}
        L = (A_2 \setminus \{i : \pi''(x^{\tau\dagger})(i) = 1\}).
        \end{align*}
        By a similar argument as in \Cref{lem:updated-indices-cmd}, we have
        \begin{align*}
        \sigma_0 =_{(A_1{\uparrow})^c} \sigma_0'',
        \quad
        \sigma_1 =_{(A_1{\uparrow})^c} \sigma_1'',
        \quad \text{and} \quad
        \dom(\pi_0''(x^{\tau\dagger})) \subseteq A_1{\downarrow}.
        \end{align*}
        Specifically, for $i \in A_2$, since $i \notin \dom(\pi_0''(x^{\tau\dagger}))$, we have
        \begin{align*}
        \pi'(x^{\tau\dagger})(i) = 1 \iff \pi''(x^{\tau\dagger})(i) = 1,
        \end{align*}
        which gives
        \begin{align*}
        L = (A_2 \setminus \{i : \pi'(x^{\tau\dagger})(i) = 1\})
        \subseteq (A \setminus \{i : \pi'(x^{\tau\dagger})(i) = 1\}).
        \end{align*}
        Since $\fixcheck(\sigma_0, \sigma_1, \pi', A)$, we have
        \begin{align*}
        \sigma_0(x^{\tau\dagger}) =_L \sigma_1(x^{\tau\dagger}).
        \end{align*}
        Also, since $L \subseteq (A_1{\uparrow})^c$, we have
        \begin{align*}
        \sigma_0(x^{\tau\dagger}) =_L \sigma_0''(x^{\tau\dagger}),
        \quad \text{and} \quad
        \sigma_1(x^{\tau\dagger}) =_L \sigma_1''(x^{\tau\dagger}).
        \end{align*}
        Together, we have
        \begin{align*}
        \sigma_0''(x^{\tau\dagger}) =_L \sigma_1''(x^{\tau\dagger}),
        \end{align*}
        which implies $\fixcheck(\sigma_0'', \sigma_1'', \pi'', A_2) = 1$.
        Combining two results on $A_1$ and $A_2$ gives
        $\fixcheck(\sigma_0'', \sigma_1'', \pi'', A) = 1$, as claimed.
        Now, since $\pi_0' \leq \pi''[\pi_0']$, by the induction hypothesis for $C_2$, we have
        \begin{align*}
        \fixcheck(\sigma_0', \sigma_1', \pi''', A_2) = 1,
        \quad
        \pi_0' = \pi_1'
        \quad
        T_0' = T_1'
        \end{align*}
        where $\pi''' = \pi''[\pi_0'] \setminus \pi_0'$.
        We claim $\fixcheck(\sigma_0', \sigma_1', \pi''', A) = 1$.
        To see this, let $x^{\tau\dagger} \in \Var$, and
        \begin{align*}
        L' = (A_1 \setminus \{i : \pi'''(x^{\tau\dagger})(i) = 1\}).
        \end{align*}
        By a similar argument as in \Cref{lem:updated-indices-cmd}, we have
        \begin{align*}
        \sigma_0'' =_{(A_2{\uparrow})^c} \sigma_0',
        \quad
        \sigma_1'' =_{(A_2{\uparrow})^c} \sigma_1',
        \quad \text{and} \quad
        \dom(\pi_0'(x^{\tau\dagger})) \subseteq A_2{\downarrow}.
        \end{align*}
        Specifically, for $i \in A_1$, since $i \notin \dom(\pi_0'(x^{\tau\dagger}))$, we have
        \begin{align*}
        \pi''(x^{\tau\dagger})(i) = 1 \iff \pi'''(x^{\tau\dagger})(i) = 1,
        \end{align*}
        which gives
        \begin{align*}
        L' = (A_1 \setminus \{i : \pi''(x^{\tau\dagger})(i) = 1\})
        \subseteq (A \setminus \{i : \pi''(x^{\tau\dagger})(i) = 1\}).
        \end{align*}
        Since $\fixcheck(\sigma_0'', \sigma_1'', \pi'', A)$, we have
        \begin{align*}
        \sigma_0''(x^{\tau\dagger}) =_{L'} \sigma_1''(x^{\tau\dagger}).
        \end{align*}
        Also, since $L' \subseteq (A_2{\uparrow})^c$, we have
        \begin{align*}
        \sigma_0''(x^{\tau\dagger}) =_{L'} \sigma_0'(x^{\tau\dagger}),
        \quad \text{and} \quad
        \sigma_1''(x^{\tau\dagger}) =_{L'} \sigma_1'(x^{\tau\dagger}).
        \end{align*}
        Together, we have
        \begin{align*}
        \sigma_0'(x^{\tau\dagger}) =_{L'} \sigma_1'(x^{\tau\dagger}),
        \end{align*}
        which implies $\fixcheck(\sigma_0', \sigma_1', \pi''', A_1) = 1$.
        Combining two results on $A_2$ and $A_1$ gives
        $\fixcheck(\sigma_0', \sigma_1', \pi''', A) = 1$, as claimed.
        Finally, simple calculations give
        \begin{align*}
        \fixcheck(\sigma_0', \sigma_1', \pi \setminus \pi_0, A) = 1,
        \quad
        \pi_0 = \pi_1,
        \quad \text{and} \quad
        T_0 = T_1
        \end{align*}
        since $(\pi \setminus \pi_0)
        = (\pi \setminus (\pi_\emptyset[h_0][\pi_0''][\pi_0']))
        = (((\pi \setminus \pi_\emptyset[h_0])[\pi_0''] \setminus \pi_0'')[\pi_0'] \setminus \pi_0')
        = \pi'''$.
    \item {\bf Case of $C \equiv (\code{extended\_loop\_with\_shift}(\alpha, n_+))$}: \\
        By the semantics, for $k \in \{0, \ldots, m\}$ and $0 \le m \le n_+{-}1$,
        \begin{align*}
        C, D, \sigma_{0, k}\langle\rho_{\alpha}\rangle, A' \Downarrowtt \sigma_{0, k+1}, \pi_{0, k+1}, T_{0, k+1},
        \quad
        C, D, \sigma_{1, k}\langle\rho_{\alpha}\rangle, A' \Downarrowtt \sigma_{1, k+1}, \pi_{1, k+1}, T_{1, k+1},
        \end{align*}
        where $\sigma_0 = \sigma_{0, 0}$ and $\sigma_1 = \sigma_{1, 0}$.
        We define
        \begin{align*}
        \pi'_{0,k+1} = \pi_{0,k+1}\langle\rho_{\alpha}\rangle^{-(k+1)}, \quad
        \pi''_{0, 0} = \pi_\emptyset, \quad
        \pi''_{0, k+1} = \pi''_{0, k}[\pi'_{0,k+1}], \quad
        \pi_0 = \pi_{0, m+1}''|_A.
        \end{align*}
        We claim that
        \begin{align*}
        \fixcheck(\sigma_{0, \ell}, \sigma_{1, \ell}, (\pi[\pi_{0, \ell}''] \setminus \pi_{0,\ell}'')\langle\rho_{\alpha}\rangle^\ell, A') = 1
        \quad
        \text{for } \ell \in \{0, \ldots, m+1\}.
        \end{align*}
        If it holds, then we have
        \begin{align*}
        \fixcheck(\sigma_{0, m+1}, \sigma_{1, m+1}, (\pi[\pi_{0, m+1}''] \setminus \pi_{0,m+1}'')\langle\rho_{\alpha}\rangle^{m+1}, A') = 1,
        \end{align*}
        which implies
        \begin{align*}
        \fixcheck(\sigma_{0, m+1}\langle\rho\rangle, \sigma_{1, m+1}\langle\rho\rangle, (\pi[\pi_{0, m+1}''] \setminus \pi_{0,m+1}''))\langle\rho_{\alpha}\rangle^{m+1}\langle\rho\rangle, A') = 1.
        \end{align*}
        Here, $\sigma_{0, m+1}\langle\rho\rangle = \sigma_0'$ and $\sigma_{1, m+1}\langle\rho\rangle = \sigma_1'$.
        Also,
        \begin{align*}
        (\pi[\pi_{0, m+1}''] \setminus \pi_{0,m+1}'')\langle\rho_{\alpha}\rangle^{m+1}\langle\rho\rangle 
        &= \pi \setminus \pi_{0,m+1}''|_A \\
        &= \pi \setminus \pi_0.
        \end{align*}
        Hence, we have $\fixcheck(\sigma_0', \sigma_1', \pi \setminus \pi_0, A') = 1$, and
        $\fixcheck(\sigma_0', \sigma_1', \pi \setminus \pi_0, A) = 1$.
        Now, we will prove the claim. If $\ell = 0$, it reduces to $\fixcheck(\sigma_0, \sigma_1, \pi, A') = 1$,
        which is true because $\fixcheck(\sigma_0, \sigma_1, \pi, A) = 1$, and $\sigma_0$ and $\sigma_1$ are $A$-states.
        Suppose the claim holds for $\ell \in \{0, \ldots, m\}$.
        Let $\pi^\ell = \pi[\pi_{0, \ell}'']\setminus \pi_{0, \ell}''$. Then,
        \begin{align*}
        \fixcheck(\sigma_{0, \ell}\langle\rho_{\alpha}\rangle, \sigma_{1, \ell}\langle\rho_{\alpha}\rangle, \pi^\ell\langle\rho_{\alpha}\rangle^{\ell+1}, A') = 1.
        \end{align*}
        By the induction hypothesis for $C$, we have 
        \begin{align*}
        \fixcheck(\sigma_{0, \ell+1}, \sigma_{1, \ell+1}, (\pi^\ell\langle\rho_{\alpha}\rangle^{\ell+1})[\pi_{0, \ell+1}] \setminus \pi_{0, \ell+1}, A') = 1.
        \end{align*}
        Since $\dom(\pi_{0, \ell+1}) \subseteq A'$, we have $\pi_{0, \ell+1}\langle\rho_{\alpha}\rangle^{-(\ell+1)}\langle\rho_{\alpha}\rangle^{\ell+1} \le \pi_{0, \ell+1}$.
        Thus,
        \begin{align*}
        (\pi^\ell\langle\rho_{\alpha}\rangle^{\ell+1})[\pi_{0, \ell+1}] \setminus \pi_{0, \ell+1}
        &= (\pi^\ell\langle\rho_{\alpha}\rangle^{\ell+1})[\pi_{0, \ell+1}\langle\rho_{\alpha}\rangle^{-(\ell+1)}\langle\rho_{\alpha}\rangle^{\ell+1}] \setminus \pi_{0, \ell+1}\langle\rho_{\alpha}\rangle^{-(\ell+1)}\langle\rho_{\alpha}\rangle^{\ell+1} \\
        &= (\pi^\ell[\pi_{0, \ell+1}\langle\rho_{\alpha}\rangle^{-(\ell+1)}] \setminus \pi_{0, \ell+1}\langle\rho_{\alpha}\rangle^{-(\ell+1)})\langle\rho_{\alpha}\rangle^{\ell+1} \\
        &= (\pi^\ell[\pi_{0, \ell+1}'] \setminus \pi_{0, \ell+1}')\langle\rho_{\alpha}\rangle^{\ell+1} \\
        &= ((\pi[\pi_{0, \ell}''] \setminus \pi_{0, \ell}'')[\pi_{0, \ell+1}'] \setminus \pi_{0, \ell+1}')\langle\rho_{\alpha}\rangle^{\ell+1} \\
        &= (\pi[\pi_{0, \ell}''[\pi_{0, \ell+1}']] \setminus (\pi_{0, \ell}''[\pi_{0, \ell+1}']))\langle\rho_{\alpha}\rangle^{\ell+1} \\
        &= (\pi[\pi_{0, \ell+1}''] \setminus \pi_{0, \ell+1}'')\langle\rho_{\alpha}\rangle^{\ell+1} \\
        &= \pi^{\ell+1}\langle\rho_{\alpha}\rangle^{\ell+1},
        \end{align*}
        which gives 
        \begin{align*}
        \fixcheck(\sigma_{0, \ell+1}, \sigma_{1, \ell+1}, \pi^{\ell+1}\langle\rho_{\alpha}\rangle^{\ell+1}, A') = 1,
        \end{align*}
        as claimed.
    \end{itemize}
\end{proof}

Let $C$ be a command in the relaxed target language.
We define the translation of $C$ to a command $\underline{C}$ in the target language as follows:
\begin{align*}
  \underline{x^\lreal := \code{fetch}(I)} & {}\;\equiv\; x^{\lreal} := \code{fetch}(I), \\
  \underline{\code{score}(E)} & {}\;\equiv\; \code{score}(E), \\
  \underline{x^\lintt := Z} & {}\;\equiv\; x^{\lintt} := Z, \\
  \underline{x^\lreal := E} & {}\;\equiv\; x^{\lreal} := E, \\
  \underline{\code{skip}} & {}\;\equiv\; \code{skip}, \\
  \underline{\code{ifz}\ Z\ C_1\ C_2} & {}\;\equiv\; \code{ifz}\ Z\ \underline{C_1}\ \underline{C_2}, \\
  \underline{C_1; C_2} & {}\;\equiv\; \underline{C_1}; \underline{C_2}, \\
  \underline{\code{for}\ x^\lintt \ \code{in} \ \code{range}(n)\ \code{do}\ C_1} & {}\;\equiv\; \code{for}\ x^\lintt \ \code{in} \ \code{range}(n)\ \code{do}\ \underline{C_1}, \\
  \underline{x^{\lintt} := \code{lookup\_index}(\alpha)} & {}\;\equiv\; x^{\lintt} := \code{lookup\_index}(\alpha), \\
  \underline{\code{extended\_loop\_with\_shift(\alpha, n)}\ C_1} & {}\;\equiv\;
  \code{extend\_index} \{ \code{loop\_fixpt\_noacc}(n)\ \{ \code{shift}(\alpha); \underline{C_1} \} \}.
\end{align*}

The following theorem states that the semantics of a command in the relaxed target language is equivalent to that of its translation in the target language.
\begin{theorem}
\label{thm:relaxed-fixed-point-soundness}
Let $C$ be a command in the relaxed target language, $D \in \RDB$, $\sigma, \sigma' \in \State_{\textit{tgt}}$,
$A \in \FAntiChain$, and $T \in \Tensor_{\R}$.
Let $\underline{C}$ be the translation of $C$ to a command in the target language.
Then,
\begin{align*}
\underline{C}, D, \sigma, A \Downarrowt \sigma', T
\quad\text{if and only if}\quad
C, D, \sigma, A \Downarrowtt \sigma', \pi, T
\quad \text{for some $\pi \in \Flag$}.
\end{align*}
\end{theorem}

\begin{proof}
The only non-trivial case is when $C$ is of the form
\begin{align*}
C \equiv (\code{extended\_loop\_with\_shift}(\alpha, n)\ C_1),
\end{align*}
and it early terminates due to the fixed-point condition.
We use the notations in the semantics of the relaxed target language. Suppose
\begin{align*}
    C, D, \sigma_\ell\langle\rho_{\alpha}\rangle, A' \Downarrowtt \sigma_{\ell+1}, \pi_{\ell+1}, T_{\ell+1},
    \quad
    &\fixcheck(\sigma_\ell\langle\rho_{\alpha}\rangle, \sigma_{\ell+1}\langle\rho_{\alpha}\rangle, \pi_{\ell+1}, A') = 0,
    \\
    C, D, \sigma_m\langle\rho_{\alpha}\rangle, A' \Downarrowtt \sigma_{m+1}, \pi_{m+1}, T_{m+1},
    \quad
    &\fixcheck(\sigma_m\langle\rho_{\alpha}\rangle, \sigma_{m+1}\langle\rho_{\alpha}\rangle, \pi_{m+1}, A') = 1.
\end{align*}
for $\ell \in \{0, \ldots, m-1\}$ and $0 \le m < n_+{-}1$.
By \Cref{lem:relaxed-fixed-point-command},
\begin{align*}
C, D, \sigma_{m+1}\langle\rho_{\alpha}\rangle, A', \Downarrowtt \sigma_{m+2}, \pi_{m+2}, T_{m+2}
\implies
&\fixcheck(\sigma_{m+1}, \sigma_{m+2}, \pi_\emptyset, A') = 1, \\
&\pi_{m+2} = \pi_{m+1}, \quad T_{m+2} = T_{m+1}.
\end{align*}
But $\fixcheck(\sigma_{m+1}, \sigma_{m+2}, \pi_\emptyset, A') = 1$ implies $\sigma_{m+1} = \sigma_{m+2}$
because they are $A'$-states.
This is the fixed-point condition in the target language, so they are semantically equivalent.
\end{proof}
